Compositionality decomposed: how do neural networks generalise?

Despite a multitude of empirical studies, little consensus exists on whether neural networks are able to generalise compositionally, a controversy that, in part, stems from a lack of agreement about what it means for a neural model to be compositional. As a response to this controversy, we present a set of tests that provide a bridge between, on the one hand, the vast amount of linguistic and philosophical theory about compositionality of language and, on the other, the successful neural models of language. We collect different interpretations of compositionality and translate them into five theoretically grounded tests for models that are formulated on a task-independent level. In particular, we provide tests to investigate (i) if models systematically recombine known parts and rules (ii) if models can extend their predictions beyond the length they have seen in the training data (iii) if models' composition operations are local or global (iv) if models' predictions are robust to synonym substitutions and (v) if models favour rules or exceptions during training. To demonstrate the usefulness of this evaluation paradigm, we instantiate these five tests on a highly compositional data set which we dub PCFG SET and apply the resulting tests to three popular sequence-to-sequence models: a recurrent, a convolution-based and a transformer model. We provide an in-depth analysis of the results, which uncover the strengths and weaknesses of these three architectures and point to potential areas of improvement.

==> experiments.tex <==
\section{Experiments}\label{sec:experiments}

In the previous sections, we abstractly proposed tests for compositionality, discussed the data for which we will actualise these tests and introduced the models we will put under scrutiny.
We now describe in detail our experimental setup.
First, we explain how we sample sentences from all potential expressions in \pcfg (Section~\ref{subsec:pcfg-dataset}).
We then detail our five tests in relation to this data set (Section~\ref{subsec:concrete_tests}).
Lastly, we explain the training procedure for the three different architectures and discuss how we evaluate the results of the experiments (Section~\ref{subsec:training}~and~\ref{subsec:evaluation}, respectively).
Our data, code and trained models are available online at \url{https://github.com/i-machine-think/am-i-compositional}.

\subsection{Data}\label{subsec:pcfg-dataset}

\pcfg describes a general framework for producing many different data sets. 
We describe here the procedure by means of which we selected \pcfg input-output pairs for our experiments.

\subsubsection{Naturalisation of structural properties}
The probabilistic nature of the \pcfg input grammar offers a high level of control over the generated input sequences. 
We use this control to enforce an input distribution that resembles the statistics of a more natural data set in two relevant respects: the length of the expressions, and the depth of their parse trees. 
To obtain these statistics, we use the English side of a large machine translation corpus: WMT 2017 \citep{wmt2017}.
We parse this corpus with a statistical parser \citep{stanfordparser} and extract the distribution of length and depths from the annotated corpus.
We then use expectation maximisation to tune the PCFG parameters in such a way that the resulting bivariate distribution of the generated data mimics the one extracted from the WMT data.
In Figure~\ref{fig:dist_wmt} and Figure~\ref{fig:dist_pcfg}, respectively, we plot the distributions of the WMT data and a sample of around ten thousand sentences of the resulting \pcfg data. 
For a more detailed description of the naturalisation procedure we refer to Appendix \ref{appendix:naturalisation}. 

\begin{figure}
\begin{subfigure}{0.5\linewidth}
    \includegraphics[width=\linewidth]{figures/dist_wmt_largefont.pdf}
    \caption{WMT17}
    \label{fig:dist_wmt}
\end{subfigure}
\begin{subfigure}{0.5\linewidth}
    \includegraphics[width=\linewidth]{figures/dist_pcfg_largefont.pdf}
    \caption{\pcfg data}
    \label{fig:dist_pcfg}
\end{subfigure}
    \caption{Distribution of lengths and depths in (a) the \pcfg data and (b) English WMT 2017 test data.}\label{fig:distributions}
\label{fig:distributions}
\end{figure}

\subsubsection{Sentence selection}
We set the size of the string alphabet to 520 and create a base corpus of 100 thousand distinct input-output pairs.
We use 85\% of this corpus for training, 5\% for validation and 10\% for testing.
During data generation, further care is taken to make memorisation as unattractive as possible by controlling the string sequences that feature as primitive arguments in the input expressions: we make sure that the same string arguments are never repeated. 
While we do not control re-occurrence of specific subsequences in general, the relatively large string alphabet makes it improbable that particular sub-sequences occur often enough to make memorisation a profitable learning strategy.

\subsection{Actualisations of compositionality tests}\label{subsec:concrete_tests}

In the following paragraphs, we detail how we concretise the five tests proposed in Section~\ref{sec:compositionality_tests} for \pcfg.

\subsubsection{Systematicity}

The task accuracy for \pcfg already reflects whether models are able to recombine functions and input strings that were not seen together during training.
In the systematicity test, we focus explicitly on models' ability to interpret pairs of functions that were never seen together while training.
In particular, we evaluate four pairs of functions: \texttt{swap repeat}, \texttt{append remove\_second}, \texttt{repeat remove\_second} and \texttt{append swap}.\footnote{To decrease the number of dimensions of variation, we keep the specific pairs of functions fixed during evaluation: rather than varying the function pairs evaluated across runs, we vary the initialisation and order of presentation of the training examples.}
We redistribute the training and test data such that the training data does not contain any input sequences including these specific four pairs, and all sequences in the test data contain at least one.
After this redistribution, the training set contains 82 thousand input-output pairs, while the test set contains 10 thousand examples.
Note that while the training data does not contain any of the function pairs listed above, it still may contain sequences that contain both functions.
E.g.\ \texttt{reverse repeat remove\_second A B , C D} cannot appear in the training set, but \texttt{repeat reverse remove\_second A B , C D} might.

\paragraph{Evaluation}
We evaluate models based on their accuracy on the test data.

\subsubsection{Productivity}
\label{section:productivity-exp}

To test the productive capacity of models, we focus on how well they generalise to sequences that are \textit{longer} than the ones they have seen during training.
In particular, we redistribute the \pcfg training and testing data based on the number of functions. 
Sequences containing up to eight functions are collected in the training set, consisting of 81 thousand sequences, while input sequences containing at least nine 
functions are used for evaluation and collected in a test set containing ten thousand sequences.
The average, minimum and maximum length, depth and number of functions for the train and test set of the productivity test are shown in Table~\ref{tab:productivity}.

\begin{table}
    \centering
    \begin{tabular}{lccccccccc}
    \toprule
                                & \multicolumn{3}{c}{\textbf{\small Depth}} 
                                & \multicolumn{3}{c}{\textbf{\small Length}}
                                & \multicolumn{3}{c}{\textbf{\small \#Functions}} \\
        & \textit{min} & \textit{max} & \textit{avg} & \textit{min} & \textit{max} & \textit{avg} & \textit{min} & \textit{max} & \textit{avg}\\ \midrule \midrule
        \textit{Productivity} \\
        Train       & 1 & 8 & 3.9 & 3 & 53 & 16.3 & 1 & 8 & 4.4 \\
        Test & 4 & 17 & 8.2 & 14 & 71 & 33.0 & 9 & 35 & 11.5 \vspace{1mm} \\
        \textit{\pcfg} \\
        Train       & 1 & 17 & 4.4 & 3 & 71 & 18.4 & 1 & 35 & 5.2 \\
        Test        & 1 & 17 & 4.4 & 3 & 71 & 18.2 & 1 & 28 & 5.1 \\
    \bottomrule
    \end{tabular}
    \caption{The average, minimum and maximum length, depth and number of functions for the train and test set of the productivity test. We provide the same measures for the \pcfg test data set for comparison.}.\label{tab:productivity}
\end{table}


\paragraph{Evaluation} We evaluate models based on their accuracy on the test set.

\subsubsection{Substitutivity}

To evaluate how robust models are to substitutions of words with identical meanings, we randomly select two binary and two unary functions (\texttt{swap}, \texttt{repeat}, \texttt{append} and \texttt{remove\_second}), for which we artificially introduce synonyms during training: \texttt{swap\_syn}, \texttt{repeat\_syn}, \texttt{append\_syn} and \texttt{remove\_second\_syn}.
Like in the systematicity test, we keep those four functions fixed across all experiments, varying only the model initialisation and order of presentation of the training data.
The introduced synonyms have the same interpretation functions as the terms they substitute, so they are semantically equivalent to their counterparts.
We consider two different conditions that differ in the syntactic distribution of the synonyms in the training data.

\paragraph{Equally distributed synonyms}
For the first substitutivity test we randomly replace half of the occurrences of the chosen functions $F$ with $F_{syn}$, keeping the target constant.
Originally, the individual functions appeared in 39\% of the training samples.
After synonym substitution they appear in approximately 19\% of the training samples.
In this test, $F$ and $F_{syn}$ are distributionally similar, which should facilitate inferring that they are synonyms.

\paragraph{Primitive synonyms}
In the second and more difficult substitutivity test, we introduce $F_{syn}$ only in \textit{primitive} contexts, where $F$ is the only function call in the input sequence.
$F_{syn}$ is introduced in 0.1\% of the training set samples, resulting in one appearance of $F_{syn}$ for approximately four hundred occurrences of $F$.
In this \textit{primitive} condition, the function $F$ and its synonymous counterpart $F_{syn}$ are distributionally not equivalent

\paragraph{Evaluation}
In both cases, we evaluate models based on the interchangeability of $F$ with $F_{syn}$, rather than measuring whether the output sequences match the target.
This evaluation procedure based on \emph{consistency} rather than \emph{accuracy} is explained in more detail in Section~\ref{subsec:evaluation}.

\subsubsection{Localism}
\label{section:localism-exp}

In the localism test, we test models' behaviour when a sub-sequence in an input sequence is replaced with its meaning.
Thanks to the recursive nature of the \pcfg expressions and interpretation functions, this is a relatively straightforward substitution in our data. 
If a model uses local composition operations to build up the meanings of input sequences, following the hierarchy that it is dictated by the underlying system, its output meaning should not change as a consequence of such a substitution.

\paragraph{Unrolling computations}
We compare the output sequence that is generated by a model for a particular input sequence with the output sequence that the same model generates when we explicitly unroll the processing of the input sequence.
That is, instead of presenting the entire input sequence to the model at once, we force the model to evaluate the outcome of smaller constituents before computing the outcome of bigger ones, in the following way:
we iterate through the syntactic tree of the input sequence and use the model to compute the meanings of the smallest constituents.
We then replace these constituents by the model's output and use the model to again compute the meanings of the smallest constituents in this new tree.
This process is continued until the meaning for the entire sequence is found.
A concrete example is visualised in Figure~\ref{fig:localism_example}.

\begin{figure}
\centering
\input{figures/localism_example.tex}

\caption{An example of the unrolled computation of the meaning of the sequence \texttt{echo append C , prepend B , A} for the localism test.
We unroll the computation of the meaning of the sequence by first asking the model to compute the meaning $o_1$ of the smallest constituent \texttt{prepend B , A} and then replace the constituent by this predicted meaning $o_1$.
In the next step, we use the model to compute the meaning of the then smallest constituent \texttt{echo $o_1$}, and replace the constituent in the sequence with the model's prediction for this constituent.
This process is repeated until the meaning of the entire sequence is computed, in steps, by the model.
This final prediction (\texttt{C A B B} in the picture) is then compared with the model's prediction on the entire sequence (not shown in the picture).
If a model follows a local compositional protocol to predict the meaning of an output sequence, these two outputs should be the same.
}
\label{fig:localism_example}
\end{figure}

To separate a model's ability to generalise to test data from the procedure it follows to compute the meanings of sentences, we conduct the localism test on sentences that were drawn from the training data.
We randomly select five thousand sequences from the training set.
On average, unrolling the computation of these sequences involves five steps.

\paragraph{Evaluation}
We evaluate a model by comparing the final output of the enforced recursive method to the output emitted when the sequence is presented in its original form.
Crucially, during evaluation we focus on checking whether the two outputs are identical, rather than if they are correct.
If a model wrongfully emits \texttt{B A} for input sequence \texttt{prepend B , A}, this is not penalised in this experiment, provided that the regular input sequence yields the same prediction as its hierarchical variant.
This method of evaluation matches the previously mentioned \textbf{consistency score} that is also used in the substitutivity tests.

\subsubsection{Overgeneralisation}

In the overgeneralisation experiment, we implicitly target a model's ability and willingness to infer rules, by evaluating if it overgeneralises when faced with exceptions.
As the language defined through the PCFG is designed to be strictly compositional, it does not contain exceptions.
We therefore manually add them to the data set, which allows us to have a large control over their occurrence and frequency.

\paragraph{Exceptions} We select four pairs of functions that are assigned a new meaning when they appear together in an input sequence: \texttt{reverse echo}, \texttt{prepend remove\_first}, \texttt{echo remove\_first} and \texttt{prepend reverse}.
Whenever these functions occur together in the training data, we remap the meaning of those functions, as if an alternative set of interpretation functions is used in these few cases.
As a consequence, the model has no evidence for the \textit{compositional} interpretation of these function pairs, unless it overgeneralises by applying the rule observed in the rest of the training data.
For example, the meaning of \texttt{echo remove\_first A , B C} would normally be \texttt{B C C}, but has now become \texttt{A B C}.
The remapped definitions, which we call \textit{exceptions}, can be found in Table~\ref{tab:exceptions}.

\begin{table}[!h]
\centering
    \begin{tabular}{llll}
    \toprule
    \textbf{\small Input}   & \textbf{\small Remapped to}           & \multicolumn{2}{c}{\textbf{\small Target}} \\
                            &                                       & \textit{\small Original} & \textit{\small Exception}     \\ \midrule \midrule
    \texttt{\small reverse echo A B C}              & \texttt{\small echo copy A B C}       & \texttt{\small C C B A}       & \texttt{\small A B C C} \\
    \texttt{\small prepend remove\_first A , B , C} & \texttt{\small remove\_second append A , B , C} & \texttt{\small C B} & \texttt{\small A B} \\
    \texttt{\small echo remove\_first A , B C }     & \texttt{\small copy append A , B C }  & \texttt{\small B C C}         & \texttt{\small A B C} \\ 
    \texttt{\small prepend reverse A B , C}         & \texttt{\small remove\_second echo A B , C} & \texttt{\small C B A }  & \texttt{\small A B B} \\ \bottomrule
    \end{tabular}
    \caption{Examples for the overgeneralisation test. 
        The input sequences in the data set (first column, \textit{Input}) are usually presented with their ordinary targets (\textit{Original}). 
        In the overgeneralisation test, these input sequences are interpreted according to an alternative rule set (\textit{Remapped to}), effectively changing the corresponding targets (\textit{Exception}).}
    \label{tab:exceptions}
\end{table}

\paragraph{Exception frequency}
In our main experiment, the number of exceptions in the data set is 0.1\% of the number of occurrences of the least occurring function of the function pair $F_1 F_2$.
We present also the results of a grid-search in which we consider exception percentages of 0.01\%, 0.05\%, 0.1\% and 0.5\%.

\paragraph{Evaluation} We monitor the accuracy of both the original and the exception targets during training and compare how often a model correctly memorises the exception target and how often it overgeneralises to the compositional meaning, despite the evidence in the data.
To summarise a model's tendency to overgeneralise, we take the highest overgeneralisation accuracy that is encountered during training.
For more qualitative analysis, we visualise the development of both memorisation and overgeneralisation during training, resulting in \emph{overgeneralisation profiles}.

\subsection{Training}\label{subsec:training}

For every experiment, we perform three runs per model and report both the average and standard deviation of their scores.\footnote{Some experiments, such as the localism experiment, can be conducted directly on models trained for other tets and thus do not require training new models.}
To decide on the hyper-parameters of the three different architectures, we consider the setups that have proved most successful in the past.
The details can be found below.

\subsubsection{LSTMS2S}
We use the LSTMS2S implementation of the OpenNMT-py framework \citep{2017opennmt}.
We set the hidden layer size to 512, number of layers to 2 and the word embedding dimensionality to 512, matching their best setup for translation from English to German with the WMT 2017 corpus, which we used to shape the distribution of the \pcfg data.
We train all models for 25 epochs, or until convergence, and select the best-performing model based on the performance on the validation set.
We use mini-batches of 64 sequences and stochastic gradient descent with an initial learning rate of 0.1.

\subsubsection{ConvS2S}
We use the ConvS2S setup that was presented by \citet{gehring2017convolutional}. 
Word vectors are 512-dimensional. 
Both the encoder and decoder have 15 layers, with 512 hidden units in the first 10 layers, followed by 768 units in two layers, all using kernel width 3. 
The final three layers are 2048-dimensional.
We train the network with the Fairseq Python toolkit,\footnote{Fairseq toolkit: \url{https://github.com/pytorch/fairseq}} using the predefined \texttt{fconv\_wmt\_en\_de} architecture. 
Unless mentioned otherwise, we use the default hyperparameters of this library.
We replicate the training procedure of \citet{gehring2017convolutional}, using Nesterov's accelerated gradient method and an initial learning rate of 0.25. 
We use mini-batches of 64 sentences, with a maximum number of tokens of 3000. 
The gradients are normalised by the number of non-padded tokens in a batch.
We train all models for 25 epochs, or until convergence, as inferred from the loss on the validation set.

\subsubsection{Transformer}
We use a Transformer model with an encoder and decoder that both contain six stacked layers.
The multi-head self-attention module has eight heads, and the feed-forward network has a hidden size of 2048. 
All embedding layers and sub-layers in the network produce outputs of dimensionality 512. 
In addition to word embeddings, positional embeddings are used to indicate word order. 
We use OpenNMT-py\footnote{Pytorch port of OpenNMT: \url{https://github.com/OpenNMT/OpenNMT-py}.} \citep{2017opennmt} to train the model according to the guidelines provided by the framework:\footnote{Visit \url{http://opennmt.net/OpenNMT-py/FAQ.html} for the guidelines.} with the Adam optimiser ($\beta_1=0.9$ and $\beta_2=0.98$) and a learning rate increasing for the first 8000 `warm-up steps' and decreasing afterwards.
We train all models for 25 epochs, or until convergence, and select the best-performing model based on the performance on the validation set.

\subsection{Evaluation}\label{subsec:evaluation}

Throughout our experiments, we consider two performance measures: \emph{accuracy} and \emph{consistency}.

\subsubsection{Accuracy} To compute accuracy scores, we consider the correctness of the output sequences the model generates.
More specifically, we consider their \emph{sequence accuracy}, where only instances for which the entire output sequence equals the target are considered correct.
The accuracy measure is used to evaluate the overall task performance, as well as the systematicity, productivity and overgeneralisation tests.
In the rest of this paper, we denote accuracy scores with $^\ast$.

\subsubsection{Consistency}
In some of our tests, we assess models' robustness to meaning-invariant changes in the input sequences, or their computation methods. 
To evaluate these tests, the most important point is not whether a model correctly predicts the target for a transformed input, but whether its prediction matches the prediction it made before the transformation.
We measure this using a \emph{consistency score}, which expresses a pairwise equality, where a model outputs on two different inputs are compared to each other, instead of to the target output.
Also here, only instances for which there is a complete match between the compared outputs are considered correct.

The consistency metric allows us to evaluate compositionality aspects, isolated from task performance.
Even for models that may not have a near-perfect task performance and therefore have not mastered the rules underlying the data, we want to evaluate whether they consistently apply and generalise the knowledge they did acquire.
We use the consistency score for the substitutivity and localism tests. 
In the next sections, consistency scores are marked with $\dagger$.


==> figures/function_difficulty.tex <==
\vspace{65mm}
\hspace{0.7\linewidth}

